DMPC: A Data-and Model-Driven Approach to Predictive Control

This work presents DMPC (Data-and Model-Driven Predictive Control) to solve control problems in which some of the constraints or parts of the objective function are known, while others are entirely unknown to the controller. It is assumed that there is an exogenous ``black box'' system, e.g. a machine learning technique, that predicts the value of the unknown functions for a given trajectory. DMPC (1) provides an approach to merge both the model-based and black-box systems; (2) can cope with very little data and is sample efficient, building its solutions based on recently generated trajectories; and (3) improves its cost in each iteration until converging to an optimal trajectory, typically needing only a few trials even for nonlinear dynamics and objectives. Theoretical analysis of the algorithm is presented, proving that the quality of the trajectory does not worsen with each new iteration, as well as providing bounds on the complexity. We apply the DMPC algorithm to the motion planning of an autonomous vehicle with nonlinear dynamics.

==> ML_model.tex <==
\tikzset{
        block/.style = {draw, rectangle,
            minimum height=1cm,
            minimum width=2cm},
        input/.style = {coordinate,node distance=1cm},
        output/.style = {coordinate,node distance=3cm}%,
        %arrow/.style={draw, -latex,node distance=2cm},
        %pinstyle/.style = {pin edge={latex-, black,node distance=2cm}},
        %sum/.style = {draw, circle, node distance=1cm},
    }
\begin{tikzpicture}[auto, node distance=2cm,font=\small]
%\end{tikzpicture} 
    \node[block] (blk1) {$\mathcal{H}$};
    \node[anchor=east] (inp11) at ($(blk1.west)+(-1,0)$) {$\mathcal{X}$};
    %\node[anchor=east] (inp12) at ($(blk1.west)+(-1,-0.25)$) {Program};
    \node[anchor=west] (out1) at ($(blk1.east)+(1,0)$) {$\mathcal{Y}$};
    %\draw[->] (inp11) -- ($(blk1.south west)!(inp11)!(blk1.north west)$);
    %\draw[->] (inp12) -- ($(blk1.south west)!(inp12)!(blk1.north west)$);
    \draw[->] (inp11) -- (blk1);
    \draw[->] (blk1)  -- (out1);
    %
    %\node[block] (blk2) at ($(blk1)+(0,-2)$) {Computer};
    %\node[anchor=east] (inp21) at ($(blk2.west)+(-1,0)$) {Data};
    %\node[anchor=east] (inp22) at ($(blk2.west)+(-1,-0.25)$) {Output};
    %\node[anchor=west] (out2) at ($(blk2.east)+(1,0)$) {Program};
    %\draw[->] (inp21) -- ($(blk1.south west)!(inp21)!(blk1.north west)$);
    %%\draw[->] (inp22) -- ($(blk1.south west)!(inp22)!(blk1.north west)$);
    %\draw[->] (blk2) -- (out2);   
    \node (fex) at ($(blk1)+(-1.1,-1.7)$) {$\mathcal{H}(\mathcal{X}) :=$};
    \node[align=left,anchor=west] at ($(fex.east)+(0.,0)$) {Differential eqns\\Difference equations\\DAEs\\State machines\\$\dots$};
    %
    \node[block] (blk2) at ($(blk1)+(6,0)$)
    {$\mathcal{Z}$};
    \node[anchor=east] (inp21) at ($(blk2.west)+(-1,0)$) {$\bar{\mathcal{X}}$};
    %\node[anchor=east] (inp22) at ($(blk2.west)+(-1,-0.25)$) {Output};
    \node[anchor=west] (out2) at ($(blk2.east)+(1,0)$) {$\bar{\mathcal{Y}}$};
    %\draw[->] (inp21) -- ($(blk1.south west)!(inp21)!(blk1.north west)$);
    %\draw[->] (inp22) -- ($(blk1.south west)!(inp22)!(blk1.north west)$);
    \draw[->] (inp21) -- (blk2);
    \draw[->] (blk2) -- (out2);    
    %
    %\node[block] (blk2) at ($(blk1)+(0,-2)$) {Computer};
    %\node[anchor=east] (inp21) at ($(blk2.west)+(-1,0)$) {Data};
    %\node[anchor=east] (inp22) at ($(blk2.west)+(-1,-0.25)$) {Output};
    %\node[anchor=west] (out2) at ($(blk2.east)+(1,0)$) {Program};
    %\draw[->] (inp21) -- ($(blk1.south west)!(inp21)!(blk1.north west)$);
    %%\draw[->] (inp22) -- ($(blk1.south west)!(inp22)!(blk1.north west)$);
    %\draw[->] (blk2) -- (out2);   
    \node (gex) at ($(blk2)+(-1.1,-1.7)$) {$\mathcal{Z}(\bar{\mathcal{X}}) :=$};
    \node[align=left,anchor=west] at ($(gex.east)+(0.,0)$) {Deep neural networks \\Random forests\\Support vector machines\\Bayesian nets\\$\dots$};
\end{tikzpicture}
\begin{subfigure}[b]{.45\textwidth}    

\label{subfig:explicit}
\caption{Explicit representation of predicted behavior}
\end{subfigure}
\begin{subfigure}[b]{.45\textwidth}    

\label{subfig:implicity}
\caption{``Learned'' representation of predicted behavior}
\end{subfigure}

==> introduction_old.tex <==
Model Predictive Control (MPC) is a well-known methodology used to control complex Cyber–Physical Systems (CPS), for example autonomous vehicles, industrial control systems, robotics systems, automatic pilot avionics, and smart grids. Conceptually, MPC involves solving an optimization problem that is constrained by (among other things) the dynamics of the system, finding a set of control inputs that minimizes the cost function. Typically, MPC relies on explicit formulation of the cost function, dynamic equations, feasibility and terminal constraints, and is therefore a \textit{model-based} procedure. \cite{garcia1989model,qin2003survey,bemporad1999robust,mayne2000survey}. 

However, in some cases, the mathematical relationship between the variables and parameters are not known either entirely or partially, and creating such a model is often cost and time prohibitive \cite{sturzenegger2015model}. One approach to overcoming this problem is to create models using historical data available from the system and embed it in the MPC and implement the optimization on the constructed model. For instance, in \cite{behl2016dr,smarra2020data} the authors propose a methodology using Regression Trees and Random Forests to build a dynamical model of a large-scale energy management system using available data. Subsequently, they apply MPC to optimize the constructed model. 

Another approach is leveraging model-based Reinforcement Learning (RL) which have shown promise in efficiently extracting information from data comparing to the model-free techniques of RL, such as Q-learning or TD-learning. Nevertheless, reinforcement learning algorithms are data inefficient and require a significant number of trials to learn even a simple task \cite{deisenroth2011pilco}. A Gaussian Processes (GPs) approach as a non-parametric method has been used to learn the dynamics of the system in \cite{deisenroth2011pilco}, and later improved in \cite{kamthe2017data} to handle the system constraints. Their new approach does not require a parametrized policy , unlike PILCO (probabilistic inference for learning control), which often needs to specify hundreds of parameters.

In this work, we assume that the dynamics of the system is available in the form of an explicit model, but there is an unknown function of the states, control inputs of the system and external disturbances that affects the performance index or feasible solution space. Also, it is assumed that there is a data-driven system which could be characterized using, for example, an appropriate machine learning framework, that is built to predict the value of this unknown function for a specific trajectory. In all of the aforementioned papers, the learning process can be completed offline and the obtained model be implemented in an MPC formulation to run the algorithm online. In that context, a large running time during training to build models is not necessarily restrictive. However, the existence of the disturbance makes the model predicted by GPs too complex to be involved in the model and then optimized. This is because disturbances require a significant increase the amount of training data necessary to fully explore the (disturbed) solution space effectively. As the most prominent weakness of standard GP is suffering from a cubic time complexity $O(n^3)$ ($n$ is training points) due to the inversion and determinant of the $n \times n$ kernel matrix, increasing the number of training data is not computationally affordable \cite{liu2020gaussian}.

We present a technique based on Iterative Learning Control (ILC) that can incorporate an unknown cost function in MPC  to generate the optimal trajectory in a few trials. The algorithm starts from a given initial trajectory and improves it by learning from each iteration until converging to an optimal solution. Iterative Learning Control is typically applied for systems that repeat the same operation under the same conditions and enables the controller to learn from  previous executions (iterations) to improve its closed-loop reference tracking performance \cite{bristow2006survey,wang2009survey}.  Traditionally, the focus of ILC is to generate a feed-forward control that minimizes deviation from a specific reference as  an error signal  or reject a repeating disturbance in the systems that execute a single repeated task \cite{lee2007iterative}.

To apply the constraints on the states of the system and control inputs, ILC was developed as as an MPC formulation in \cite{lee2000convergence} for a batch processing. They propose a time varying system in which an error signal is incorporated as a dynamic memory of executed batches. They show that this error becomes smaller by increasing the number of iterations. A similar approach has been conducted in \cite{lee1997model} for nonlinear batch to achieve perfect tracking in square systems. In all of the described work in ILC it is assumed that there is a reference signal available for the controller. In \cite{rosolia2017learning} the presented framework does not require a reference signal, which can be challenging to find for a system with complex environments and nonlinear dynamics. The algorithm, called Learning Model Predictive Control (LMPC), assumes that the initial conditions, the constraints, and the performance index stay consistent. They show that the cost function does not increase with each iteration and also prove the recursive feasibility of the algorithm \cite{rosolia2018learning,brunner2017repetitive,rosolia2017robust}. However, none of these works incorporate data-driven systems or subsets of variables, and they assume that all components of the model can be explicitly formulated a priori. LMPC is a so-called ``white box'' approach. 

 An application for this problem can be found in Connected Autonomous Vehicles (CAVs), in which a vehicle shares its optimal trajectory with another vehicle in the platoon, and accordingly the controller of the other vehicle generates an optimal and safe trajectory. The vehicles in the platoon use a wireless communication channel to share the information of their trajectory, which does not operate perfectly and there is a delay and uncertainty in the channel. The length of delay in the wireless channel is an unknown function of the states of two communicating vehicles and surrounding environment (e.g infrastructures, other approaching vehicles and etc.). We have addressed this problem in \cite{9029830} and proposed a LMPC method to solve it, where the controller updates the model at each iteration to explore the areas of uncertainty with respect to the wireless channel and gradually converges to the optimal trajectory. The problem with this approach is that it can only handle a very simple binary environment (area with zero or infinite delay) with a rectangular shape. Increasing the complexity of area, both in terms of its topology and distribution of delay, is a demanding process. Also, it is computationally expensive and requires knowledge from the environment to build the part of the initial model that deals with the areas of disconnection in the wireless channel. These problems prevent the algorithm to be generalized to other applications.

Generally, the main challenge this paper seeks to address involves accounting for the interconnection between the known functions and unknown functions, a setting that is increasingly prevalent in control applications. Model-driven variables are a set of decision variables with behaviour and relations that can be described analytically in the model (e.g. system dynamics). However, closed-form models are not possible, or computationally affordable, for data-driven systems and these behaviors are typically predicted by using, for example, deep learning techniques. The learning techniques and MPC can be leveraged to predict the behaviour of the data-driven and model driven systems and this work develops a technique to incorporate both systems in an algorithm called Data-and Model-driven Predictive Control (DMPC).  DMPC works without a reference trajectory but it needs an initial trajectory to begin with. We prove that DMPC is recursively feasible at each iteration and the generated trajectories will not worsen at each iteration. This algorithm needs only few iterations to converge to a locally optimally solution and it is computationally efficient. 

==> notations.tex <==

\renewcommand{\arraystretch}{0.9}% Tighter
\begin{table}[htbp]
\centering
\caption{Main Notations}
\label{tab:table1}
\begin{tabularx}{8.5cm}{p{1.3cm} p{6.5cm}}
\toprule
\textbf{Notation} & \textbf{Meaning} \\
\midrule
$x_t$ & system state at time $t$ \\
$u_t$  & control input at time $t$ \\
$n$ & number of states in system dynamics \\
$m$ & number of control inputs in system dynamics \\
$N$ & time horizon \\
$f$ & known nonlinear map\\
$\mathcal{X}$ & feasible state vector space\\
$\mathcal{U}$ & feasible control vector space\\
$x_S$ & initial state\\
$x_F$ & final state\\
$h()$ & known function\\
$\hat{z}()$ & unknown function\\
$\mathcal{J}_{0\to\infty}$ & overall cost function\\
$j$ & iteration index\\
$\textbf{x}^{*,j}$ & optimal state vector of iteration $j$\\
$\textbf{u}^{*,j}$ & optimal control vector of iteration $j$\\
$x_t^{*,j}$ & optimal state at time $t$ and iteration $j$\\
$u_t^{*,j}$ & optimal control input at time $t$ and iteration $j$\\
$q^{j-1}()$ & cost-to-go value for each state at iteration $j-1$\\
$\textbf{q}^{j-1}$ & cost-to-go vector at iteration $j-1$\\
$\textbf{x}_{t:t+N|t}^{j}$ & optimal state from $t$ to $t+N$ estimated at $t$\\
$\textbf{u}_{t:t+N|t}^{j}$ & optimal control from $t$ to $t+N$ estimated at $t$\\
$u_{t+N-1|t}^{j}$ & optimal control at step $t+k$ estimated at $t$\\
$x_{t+N|t}^{j}$ & optimal state at step $t+k$ estimated at $t$\\
$x_F$ & final state\\
$h()$ & known function\\
$\hat{z}()$ & unknown function\\
$\mathcal{J}_{0\to\infty}$ & overall cost function\\
$j$ & iteration index\\
$\textbf{x}^{*,j}$ & optimal state vector of iteration $j$\\
$\textbf{u}^{*,j}$ & optimal control vector of iteration $j$\\
$x_t^{*,j}$ & optimum state at time $t$ and iteration $j$\\
$u_t^{*,j}$ & optimum control at time $t$ and iteration $j$\\
$q^{j-1}()$ & cost-to-go value for each state at iteration $j-1$\\
$\textbf{q}^{j-1}$ & cost-to-go vector at iteration $j-1$\\
$\textbf{u}_{t:t+N|t}^{j}$ & optimal control from $t$ to $t+N$ estimated at $t$\\
$\textbf{x}_{t:t+N|t}^{j}$ & optimal state from $t$ to $t+N$ estimated at $t$\\
$u_{t+N-1|t}^{j}$ & optimal control at step $t+k$ estimated at $t$\\
$x_{t+N|t}^{j}$ & optimal state at step $t+k$ estimated at $t$\\
$Reach(\mathcal{B})$ & one-step reachable set $\mathcal{B}$\\
$\mathcal{R}_N(\mathcal{X}_0)$ & $N$-step reachable set $\mathcal{X}_0$\\
$\mathcal{S}_t^j$ & $N$-step reachable states of iteration $j$ at time $t$\\
$\mathcal{C}$ & control invariant set\\
$\textit{s}_t^{i,j}$ & $i^{th}$ state in set $\mathcal{S}_t^j$\\
$\textbf{u}_{t:t+N|t}^{i,j}$ & optimal policy to reach terminal state $\textit{s}_t^{i,j}$\\
$\textbf{x}_{t:t+N|t}^{i,j}$ & optimal state vector from control input $\textbf{u}_{t:t+N|t}^{i,j}$\\
$\overbar{\textbf{u}}_{t:t+N|t}^j$ & optimal control vector to generate $\overbar{\textbf{x}}_{t:t+N|t}^j$\\
$\overbar{\textbf{x}}_{t:t+N|t}^j$ & optimal state vector to the best state in set $\mathcal{S}_t^j$ \\
$\mathcal{J}_{t\to t+N}^{i,j}()$ & predicted overall cost of following policy \\
$\hat{z}_{k|t}^{i,j}$ & predicted value of the unknown function following the control input $\textbf{u}_{t:t+N}^{i,j}$\\
$J_{t\to t+N}^{i,j}()$ & model-based trajectory cost from $x_t^{*,j}$ to $s_t^{i,j}$\\
$\ell(.,.)$ & alternative positive definite cost function\\
$P$ & positive semi-definite weighting matrix\\
\bottomrule
\end{tabularx}\\
\end{table}
\renewcommand{\arraystretch}{0.9}% Tighter
\begin{table}[ht!]
\begin{tabularx}{8.5cm}{p{1.3cm} p{6.5cm}}
\toprule
\textbf{Notation} & \textbf{Meaning} \\
\midrule
$R$ & positive definite weighting matrix\\
$\overbar{\mathcal{J}}_{t\to t+N}^{j}()$ & minimum overall trajectory cost from $x_t^{*,j}$ to the best terminal state in $\mathcal{S}_t^j$\\
$x_{\tau}^{*,j-1}$ & the optimal terminal state selected at the previous time step to reach from state $x^{*,j}_{t-1}$\\
$u_{\tau}^{*,j-1}$ & control input to drive the system from state $x_{\tau}^{*,j-1}$ to $x_{\tau+1}^{*,j-1}$ along $\textbf{x}^{*,j-1}$\\
$\textbf{u}_{t:t+N|t-1}^{j}$ & control to drive the system from $x^{*,j}_t$ to $x_{\tau+1}^{*,j-1}$\\
$\textbf{x}_{t:t+N|t-1}^{j}$ & trajectory obtained by applying $\textbf{u}_{t-1:t+N-1|t-1}^{j}$\\
$\mathcal{J}_{t\to t+N|t-1}^{j}$ & The overall trajectory cost from $x_{t}^{*,j}$ to $x_{\tau+1}^{*,j-1}$\\
$\mathcal{J}_{t\to t+N}^{j}()$ & the minimum trajectory cost from state $x_t^{*,j}$\\
$u_t^{*,j}$ & applied first step of optimal control policy\\
$x_{t+1}^{*,j}$ & reached state by applying control input $u_t^{*,j}$\\
$Q_t^j$ & cost to go vector of terminal states based on the current state ${x}_t^{*,j}$\\
$r$ & binary variable index\\
$\xi_r$ & $r^{th}$ binary variable\\
$\iota$ & index of selected terminal state by model (\ref{eq:Implem_DMPC_generic-model})\\
$\iota^*$ & index of best terminal state\\
$\mathrm{x}_{min}$ & lower bound for feasible state space\\
$\mathrm{x}_{max}$ & upper bound for feasible state space\\
$\mathrm{u}_{min}$ & lower bound for feasible control space\\
$\mathrm{u}_{max}$ & upper bound for feasible control space\\
${x}_t$ & $x$ coordination of the vehicle \\
${y}_t$ & $y$ coordination of the vehicle\\
${\psi}_t$ & heading angle of the vehicle\\
${v}_t$ & velocity of the vehicle\\
${\beta}_t$ & angle of the velocity vector in the vehicle\\
${\delta}_t$ & steering angle the vehicle\\
${a}_t$ & acceleration/deceleration of the vehicle\\
$\tilde{\textbf{x}}$ & training input data\\
$\hat{z}$ & training target data\\
% $\tilde{\textbf{X}}$ & matrix of training input data\\
% $\tilde{\textbf{z}}$ & vector of training target data\\
% $\tilde{\textbf{x}}_*$ & test input data\\
% $z_*$ & test target data\\
% $\sigma^2_{\varepsilon}$ & variance of noise\\
% $m()$ & mean function of $z_*$ \\
% $\sigma^2()$ & variance function of $z_*$\\
% $\textbf{K}$ & Gram matrix\\
% $k(.,.)$ & entries of $\textbf{K}$\\
% $\pmb{\mu}_{k|t}$ & mean of $\tilde{\textbf{x}}_{k|t}$\\
% $\pmb{\Sigma}_{k|t}$ & covariance of $\tilde{\textbf{x}}_{k|t}$\\
\bottomrule
\end{tabularx}\\
\end{table}


==> pseudocode_DMPC.tex <==
\begin{algorithm}%[h]
\caption{: DMPC}
\label{alg}
\begin{algorithmic}[1]
\STATE {Set $j=0$; $convergence \leftarrow 0$}
\WHILE{($!convergence$)}
\STATE {Update $j \leftarrow j+1$ and set $t=0$}
\STATE {Set $x_{0}^{*,1} \leftarrow x_S$, $\textbf{x}^0$, $\textbf{u}^0$, $\textbf{q}^0$}
\WHILE{($x_{t}^{*,j} \neq x_F$)}
\STATE {$Q^j \leftarrow \bigcup_{r=0}^{\infty}{q}^{j-1}(x_r^{*,j-1})$}
\STATE {Set $I \leftarrow \varnothing$ and $Q_t^j \leftarrow Q^j$}
\STATE {Set $\iota \leftarrow -1$, $flag \leftarrow 1$}
\WHILE{($flag$)}

\STATE {Solve IP model (\ref{eq:Implem_DMPC_generic-model})}
\STATE {Save the solution as $\mathpzc{X}=[x_t^{*,j}, \dots, x_{\iota}^{*,j-1}]$}, $\iota$ is the index of the selected terminal state, ($x_{\iota}^{*,j-1}$) from set $Q_t^j$
\STATE {Save the cost value as $J_{t\to t+N}^{j}(x_t^{*,j})$}

\IF {$(\iota \notin I)$}
\STATE {$I \leftarrow \iota \cup I$}
\STATE {Feed $\mathpzc{X}$ into the Exogenous System to receive the prediction $[\hat{z}_{t|t}^j, \dots, \hat{z}_{t+N-1|t}^j]$}
\STATE {$Q_t^j(x_{\iota}^{*,j-1}) \leftarrow Q_t^j(x_{\iota}^{*,j-1}) + \sum_{k=t}^{t+N-1}\hat{z}_{k|t}^{j}$}
\ELSE
\STATE {$\mathcal{J}_{t\to t+N}^{j}(x_t^{*,j}) \leftarrow J_{t\to t+N}^{j}(x_t^{*,j})$}
\STATE {$flag \leftarrow 0$}
\ENDIF
\ENDWHILE
\STATE {Construct $\textbf{x}_{t:t+N|t-1}^{j}$ based on equation (\ref{eq:trajectory_i_last_time_step})}
\STATE {Calculate $\mathcal{J}_{t\to t+N|t-1}^{j}(x_{t}^{*,j})$ according to (\ref{eq:secondary_traj_ii})}
\STATE {Select the best of $\mathpzc{X}$ and $\textbf{x}_{t:t+N|t-1}^{j}$ as $\textbf{x}_{t:t+N|t}^{*,j}$ based on $\mathcal{J}_{t\to t+N}^{j}(x_t^{*,j})$ and $\mathcal{J}_{t\to t+N|t-1}^{j}(x_{t}^{*,j})$}
\STATE {Apply the first control input from $\textbf{u}_{t:t+N|t}^{*,j}$}
\STATE {Update $t \leftarrow t+1$}
\ENDWHILE
\IF {$\sum_{t=0}^{\infty} |x_{t}^{*,j} - x_{t}^{*,j-1}| < \varepsilon$}
\STATE {$convergence \leftarrow 1$}
\ENDIF
\ENDWHILE
\STATE {$\textbf{x}^{*,j} = [ x_S, x_1^{*,j}, \dots , x_t^{*,j}, \dots, x_F]$ is optimal}
\end{algorithmic}
\end{algorithm}

